The Hard Positive Truth about Vision-Language Compositionality

Several benchmarks have concluded that our best vision-language models (e.g., CLIP) are lacking in compositionality. Given an image, these benchmarks probe a model's ability to identify its associated caption amongst a set of compositional distractors. In response, a surge of recent proposals show improvements by finetuning CLIP with distractors as hard negatives. Our investigations reveal that these improvements have, in fact, been significantly overstated -- because existing benchmarks do not probe whether finetuned vision-language models remain invariant to hard positives. By curating an evaluation dataset with 112,382 hard negatives and hard positives, we uncover that including hard positives decreases CLIP's performance by 12.9%, while humans perform effortlessly at 99%. CLIP finetuned with hard negatives results in an even larger decrease, up to 38.7%. With this finding, we then produce a 1,775,259 image-text training set with both hard negative and hard positive captions. By training with both, we see improvements on existing benchmarks while simultaneously improving performance on hard positives, indicating a more robust improvement in compositionality. Our work suggests the need for future research to rigorously test and improve CLIP's understanding of semantic relationships between related "positive" concepts.

==> old/abstract_v1.tex <==

Many recent works study the lack of robustness in vision-language models: specifically, showing that even powerful image-text matching models are insensitive to label-altering perturbations in the text input (``hard negatives''). 
We posit that this definition of robustness is lacking: it does not acknowledge the existence of label-\textit{retaining} perturbations (``hard positives''). 
We curate a benchmark to test two major types of hard positives, each targeting a type of hard negative finetuning popular in practice: word replacement and word swapping.
We show that existing work that attempts to improve model compositionality by training on hard negatives actually significantly reduces performance when accounting for hard positives by as much as 27 absolute points. 
% By modifying the definition of robustness to account for hard positives as well as hard negatives, 
We train a model on both hard negatives and hard positives, and show that by accounting for both, we are able to improve overall model performance on both, without sacrificing clean performance --- compared to the same model with just hard negative training, as well as compared to all existing works incorporating hard negative training. However, there is significant room for improvement compared to human performance. 

% When the definition is incomplete and we focus on fixing the problem on one side, it amplifies the issue on the other side. The key difference between this and the current story is arguing we need to redefine the notion of robustness in image-text matching and the definition has to consider both sides, and based on the new definition, we can come up with better algorithms to achieve robustness.


% Many recent works have studied the existence of ``hard negatives'' for vision-language models: specifically, showing that even powerful image-text matching models are insensitive to label-altering perturbations in the text input. 
% Several of these studies go on to finetune on these hard negatives, resulting in models that now (more frequently) appropriately change their prediction on label-altering perturbations. 
% However, what are the drawbacks of hard-negative finetuning? 
% We posit that while this finetuning increases understanding of hard negatives, it decreases understanding of hard \textit{positives}, i.e. label-retaining perturbations. 
% We curate a benchmark to test several types of hard positives, each targeting a type of hard negative finetuning that exists in practice. 
% We evaluate models with and without hard negative finetuning, and show that hard-negative finetuning indeed increases brittleness to hard positives. 
% We further explore methods to overcome this issue, finding that more comprehensive finetuning methods and model averaging improve model performance on hard negatives and hard positives \cy{remove model averaging}.


\keywords{vision-language \and fine-grained understanding \and robustness \and compositionality}

==> old/abstract_v2.tex <==

A number of recent works have concluded that our best vision-language models (\eg~CLIP) are lacking in  compositionality.
Given an image, these benchmarks probe a model's ability to identify its associated caption amongst a set of compositional distractors.
In response, a surge of recent papers show improvements by finetuning CLIP by mining distractors—\textbf{hard negatives}.
Our investigations reveal that these improvements have been overstated do not probe whether finetuned models remain invariant to \textbf{hard positives}.
We curate a probing dataset and uncover that models, which have been finetuned with hard negatives, perform significantly worse on our probe by as much as 27\%. 
With this finding, we explore the impact of finetuning CLIP models using both hard positives and negatives.
By accounting for both, we see improvements on existing benchmarks while simultaneously minimizing errors towards positives.
Our work suggests the need for further probes to rigorously test CLIP's understanding of semantic relationships between related ``positive'' concepts.

% By modifying the definition of robustness to account for hard positives as well as hard negatives, 

% When the definition is incomplete and we focus on fixing the problem on one side, it amplifies the issue on the other side. The key difference between this and the current story is arguing we need to redefine the notion of robustness in image-text matching and the definition has to consider both sides, and based on the new definition, we can come up with better algorithms to achieve robustness.


% Many recent works have studied the existence of ``hard negatives'' for vision-language models: specifically, showing that even powerful image-text matching models are insensitive to label-altering perturbations in the text input. 
% Several of these studies go on to finetune on these hard negatives, resulting in models that now (more frequently) appropriately change their prediction on label-altering perturbations. 
% However, what are the drawbacks of hard-negative finetuning? 
% We posit that while this finetuning increases understanding of hard negatives, it decreases understanding of hard \textit{positives}, i.e. label-retaining perturbations. 
% We curate a benchmark to test several types of hard positives, each targeting a type of hard negative finetuning that exists in practice. 
% We evaluate models with and without hard negative finetuning, and show that hard-negative finetuning indeed increases brittleness to hard positives. 
% We further explore methods to overcome this issue, finding that more comprehensive finetuning methods and model averaging improve model performance on hard negatives and hard positives \cy{remove model averaging}.


\keywords{vision-language models \and hard positives \and clip \and compositionality}

==> old/compo_v1.tex <==



\section{An updated definition and evaluation of compositionality}

\jy{If the overall story is about compositionality, then we should talk about it more and motivate the study using it. Right now compositionality is not mentioned in either Sec 3 4 or 5}

\jy{right now the beginning of sec 3 4 5 is not clear and convincing; I suppose a (nice) reader should be able to get the idea and be convinced by only reading the beginning of sec 3 4 5. I try to lay out the logic of first paragraph of sec 3 4 5 below}

\jy{for sec 3, "existing benchmarks evaluate compositionality by considering compositionally hard negatives only due to a fact that if a model couldn't recognize that two slightly different compositions actually correspond to different images, which means the VLM lacks the capability to distinguish different compositions and therefore lack compositional understanding. However, such an evaluation is incomplete because compositionality actually includes both 1) knowing two compositions are semantically different and 2) knowing two compositions are semantically identical. Therefore, to enable the study of 2) we propose to evaluate hard positive " }

\jy{for sec 4, "the goal of HN fine-tuning is to achieve compositionality by letting the model know certain perturbation would change the meaning of caption so that is no longer aligned with the image, in order to let model understand different compositions of basic elements matter. However, overemphasizing on HN indeed let model leans perturbations always change the meaning, overlooking the fact that sometimes they do not."}

\jy{Then for sec 5, we can say that because the reason is current learning objective is just letting model know perturbation would change meaning. So a better learning objective is to let model know when it changes. To achieve this, we explore hard positive finetuning}






% \subsection{Definition}
Consider an image $i$ and a caption $c$. The objective of an ITM model is to compute a score $s(c,i)$ that should be high if the caption accurately corresponds to the image, and low otherwise. Let us now introduce a perturbation function $\mathcal{P}$ that minimally perturbs a caption, e.g., by replacing one word in the caption with another, or by swapping two phrases within the caption. $\mathcal{P}(c)$ may still match the image (label-retaining perturbation) or may not (label-altering perturbation). 

Existing work only considers label-altering perturbations. The model is encouraged by both the evaluation and the finetuning loss to award a low ITM score to the perturbed caption, i.e., a low $s(\mathcal{P}(c), i)$. 

We posit that a more well-rounded definition of robustness accounts for label-retaining perturbations as well, i.e., recognizes that $s(\mathcal{P}(c), i)$ should be high if $\mathcal{P}(c)$ retained the meaning of the caption $c$ and low otherwise. This refined definition ensures that the ITM model is encouraged to identify \textit{when} a perturbation to a caption changes its match to an image, rather than assuming that all perturbations to a caption change its match to the image.
% acknowledges the semantic fidelity of perturbed captions that remain relevant to the image.


\subsection{Benchmarks}
\label{sec:benchmarks}
This section discusses the benchmarks we curate to test vision-language model understanding of hard positives, i.e., label-retaining perturbations to the caption. We focus on the two main types of perturbations in existing work: replacing one word or phrase in the caption; or swapping two words or phrases within the caption. To our knowledge, no other type of perturbation is nearly as well-studied. 

Each data point in these benchmarks contains one image and three captions: the original caption, a hard negative (sourced from an existing hard negative benchmark) and a hard positive (generated by us).
Figure \ref{fig:benchmarks} shows examples from our benchmarks.

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/dataset_figure.pdf}
  \caption{Our \replace and \swap evaluation sets. \replace replaces either an attribute or a relation in the original caption $c$ to obtain $c_N$ and $c_P$. \swap swaps the object-attribute associations in the original caption $c$ to obtain $c_N$ and $c_P$.}
  \label{fig:benchmarks}
\end{figure}

\subsubsection*{REPLACE}
The most popular type of hard negative considered by existing work is \replace, where one word or phrase in the caption is replaced with another in a way that changes the meaning of the caption \cite{zhao2022vl, parcalabescu-etal-2022-valse, ma2022crepe, doveh2023teaching, doveh2023dense, kamath-etal-2023-whats, kamath2023text, hendricks-nematzadeh-2021-probing}.
% VL-Checklist, VALSE, CREPE, SVLC, DAC, ControlledImCaps, WhatsUp, SVO, VSR.
To create hard positives, we replace one word or phrase in a way that does \textit{not} change the meaning of the caption. 

We begin with examples from VL-Checklist \cite{zhao2022vl}. This benchmark contains \replace hard negatives targeting either objects, attributes or relations. We focus on attributes and relations, as they have been shown to be more challenging for vision-language models to understand \cite{doveh2023teaching, doveh2023dense, hsieh2023sugarcrepe}, and select the subset of VL-Checklist based on Visual Genome \cite{krishna2017visual} to stay consistent with our \swap benchmark.
The VL-Checklist Relations benchmark has two types of relations: actions and spatial. The VL-Checklist Attributes benchmark has five types of attributes: action\footnote{The action \textit{relation} is usually a transitive verb, e.g., ``a person wearing a shirt'', whereas the action \textit{attribute} is usually an intransitive verb, e.g., ``a person standing''.}, color, material, size, and state. 

For each of these types, we collect the ten most common relations/attributes, and hand-write a fixed replacement that holds for the various word senses of each original word. If no replacement can be found, we discard the replacement. 
Finally, we replace 14 relations and 24 attributes, resulting in a benchmark of 16,868 hard positives targeting relations, and 10,575 hard positives targeting attributes, for a total of 27,443 examples. Refer to the Supplementary for further details.



For example, for the Visual Genome caption ``cutting board next to pan'', VL-Checklist constructs a hard negative by replacing the relation with an antonym: ``cutting board \textit{far from} pan''. We construct a hard positive by replacing the relation with a synonym: ``cutting board \textit{near} pan''. 
While there may be minor differences between the original and hard positive captions (e.g., ``next to'' may imply a closer spatial relation than ``near''), they are both a match for the image, while the hard negative caption is not. 


\subsubsection*{SWAP}
Another popular type of hard negative considered by existing work is \swap, where two words or phrases in a caption are swapped with each other in a way that changes the meaning of the caption \cite{yuksekgonul2023when, parcalabescu-etal-2022-valse, ma2022crepe, thrush2022winoground}. 
To create hard positives, we swap two phrases in a way that does not change the meaning of the caption.

We begin with the Visual Genome Attribution (VGA) set from the Attribute-Relation-Order benchmark \cite{yuksekgonul2023when}, which switches object-attribute associations in a Visual Genome caption to create a hard negative, e.g., ``the crouched cat and the open door'' $\xrightarrow{}$ ``the open cat and the crouched door''. 
To create a hard positive, we switch the word order while retaining the object-attribute associations, and thus retaining the meaning of the caption, e.g., ``the open door and the crouched cat''.
While there are small linguistic differences between the original and hard positive captions (e.g., people tend to describe the most salient object first), they are both a match for the image, where the hard negative caption is not. 

% The VGA dataset contains 28748 examples. 
% The captions are all programmatically generated from VG annotations and follow the format ``the \{adjective\_1\} \{noun\_1\} and the \{adjective\_2\} \{noun\_2\}'', as in the example discussed above. 
We create a hard positive for each example in the VGA dataset, resulting in a benchmark of 28,748 examples.

% Why no relation/object


==> old/intro_v1.tex <==

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/teaser.png}
  \caption{Placeholder for teaser figure.}
  \label{fig:teaser}
\end{figure}

% \section*{Notes:}
% \begin{itemize}
%     \item We should probably have the word ``robustness'' somewhere?
%     \item Trade-off between hard negatives and hard positives
% \end{itemize}

\section{Introduction}

Recent advances in image-text matching (ITM) models, such as CLIP~\cite{RadfordKHRGASAM21} and ALIGN~\cite{jia2021scaling}, have enabled the use many downstream applications ranging from zero-shot classification and retrieval~\cite{} to pushing forward the field of multimodal learning. This includes using ITM models to power various other types of vision-language models such as BLIP~\cite{li2022blip, li2023blip2}, DALL-E~\cite{ramesh2021zero, ramesh2022hierarchical, BetkerImprovingIG}, Stable Diffusion~\cite{rombach2022high}, and to curate better vision-language datasets~\cite{laion5b, gadre2023datacomp}.

% Image-text matching (ITM) models such as CLIP~\cite{RadfordKHRGASAM21} are very popular in vision-language, due to their easy scalability and high performance. They are used in a wide variety of downstream applications, from image retrieval to text-to-image generation.

However, a spate of recent works pointed out that current ITM models lack fine-grained vision-language understanding, by showing that the models are insensitive to small but semantic-altering perturbations applied to the captions~\cite{thrush2022winoground, zhao2022vl, ma2022crepe, yuksekgonul2023when, hsieh2023sugarcrepe}, wherein the models often assign higher image-text matching scores to the perturbed captions, commonly known as \textit{hard negatives}. For instance, CLIP assigns a higher image-text matching score to ``grass eating horse'' than ``horse eating grass'', for an image of the latter~\cite{yuksekgonul2023when}. 
Since then, many approaches have been proposed to fix this problem by explicitly training the models to increase their sensitivity to minimal but semantic-altering perturbations~\cite{yuksekgonul2023when, doveh2023teaching}.

Ideally, a model with true fine-grained understanding capability should not only be able to distinguish the correct caption from the semantic-altering hard negatives, it should also be able to tell when a small perturbation is in fact semantic-preserving, i.e., they should be robust to semantic-preserving perturbations.
Motivated by the robustness point of view, we note that existing hard negative based evaluations measure only the \textit{sensitivity} of the model to small perturbations---they only test if the model can distinguish correct caption from the hard negatives.
However, without measuring the models' \textit{stability} to semantic-preserving perturbations, a model attaining strong sensitivity to perturbations can in fact be poor in its generalization to semantic-preserving changes~\cite{cite}.

To more faithfully measure IMT models' fine-grained vision-language understanding capabilities, we introduce the first benchmark \bname, to the best of our knowledge, that not only tests the model's sensitivity to hard negatives but their stability to \textit{hard positives}, obtained by minimally changing the captions without altering their semantics. \cy{add examples}.

By evaluating recently introduced methods targeting to improve models' sensitivity to hard negatives on \bname, we unfortunately find that existing methods improve model performances on hard negatives at the cost of their stability on hard positives. For instance, \cy{add example and numbers}.
To mitigate this sensitivity-and-stability tradeoff, we propose a simple data-augmentation training technique wherein the models are trained simultaneously with both hard negatives and hard positives. By training the model to distinguish between semantically-preserving and -altering perturbations, we find that the technique simultaneously improves both the model's sensitivity as well as stability. \cy{add numbers}. We hope that with the more comprehensive evaluation, \bname can foster better future methods to effectively improve model's fine-grained vision-language understanding.






% \section*{Introduction v1}
% \label{sec:old-intro}
% Image-text matching (ITM) models such as CLIP are very popular in vision-language, due to their easy scalability and high performance. They are used in a wide variety of downstream applications, from image retrieval to text-to-image generation. However, a spate of recent works show that these models perform poorly on ``hard negatives'', i.e., small label-altering perturbations. For example, CLIP assigns a higher image-text matching score to ``grass eating horse'' than ``horse eating grass'', for an image of the latter. 

% Many of these works then finetune on these hard negatives, aiming to teach these models the underlying concept: how word swaps/replacements impact meaning. They show that the finetuned models now recognize that the original caption is a match for the image and the hard negative caption is not, and claim that the models now understand how word swaps/replacements impact meaning, exhibiting improved fine grained vision-language understanding.

% However, we posit that hard negatives do not teach models \textit{how} word swaps/ replacements \textit{impact} meaning – it teaches models \textit{that} word swaps/replacements \textit{change} meaning, \textit{always}. Specifically, they do not teach models when it changes meaning and when it does not, which is required to truly improve fine-grained vision-language understanding.

% To prove this, we create a benchmark of hard positives: label-\textit{retaining} perturbations to captions, targeting each of the two main types of hard negatives in existing work, word swaps and replacements. We show that models finetuned on hard negatives do not recognize etc etc, (so they didn't really learn anything and end up brittle)

% [working on this in a separate doc]

==> old/scratch.tex <==






==> tables/improved_results_a.tex <==
\begin{table}[t]
\centering
\resizebox{0.7\columnwidth}{!}{  

            \begin{tabular}{lcccc}
            \toprule
              % Model & \begin{tabular}{@{}c@{}}\texttt{Whats-} \\ \texttt{Up}\end{tabular} & \begin{tabular}{@{}c@{}}\texttt{COCO-} \\ \texttt{spatial}\end{tabular} & \begin{tabular}{@{}c@{}}\texttt{GQA-} \\ \texttt{spatial}\end{tabular} & Avg\\
               & \multicolumn{2}{c}{\texttt{REPLACE}} & \multicolumn{2}{c}{\texttt{SWAP}} \\
              Model & \hspace{5px}$c > c'$\hspace{5px} & \hspace{5px}$c, c'' > c'$\hspace{5px} & \hspace{5px}$c > c'$ \hspace{5px}& $c, c'' > c'$\\
              \midrule
              CLIP ViT-B/32 & 61.6 & 46.8 {\scriptsize\textcolor{red}{(-14.9)}}& 60.5 & 49.6 {\scriptsize\textcolor{red}{(-10.9)}} \\
              \midrule
              Our HN & 73.9 & 55.7 {\scriptsize\textcolor{red}{(-18.2)}}& 74.3 & 60.5 {\scriptsize\textcolor{red}{(-13.8)}}\\
              Our HP+HN & 69.0 & 58.0 {\scriptsize\textcolor{red}{(-11.0)}}& 73.2 & 61.1 {\scriptsize\textcolor{red}{(-12.1)}}\\
              Our HP+HN (Swap-only) & 63.9 & 51.6 {\scriptsize\textcolor{red}{(-12.3)}}& 73.0 & 61.9 {\scriptsize\textcolor{red}{(-11.2)}}\\
              Our HP+HN (Replace-only) & 70.9 & 59.0 {\scriptsize\textcolor{red}{(-11.9)}}& 69.7 & 55.6 {\scriptsize\textcolor{red}{(-14.1)}}\\
              \midrule
              Human Estimate &  & & & \\
              \bottomrule \\
            \end{tabular}
        }
\caption{Our true performance is better.
}
\label{tab:improved_results_1}
\end{table}

% {\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}}97


==> tables/improved_results_b.tex <==
\begin{table}[t]
\centering
\resizebox{0.55\columnwidth}{!}{  

            \begin{tabular}{lcc}
            \toprule
              % Model & \begin{tabular}{@{}c@{}}\texttt{Whats-} \\ \texttt{Up}\end{tabular} & \begin{tabular}{@{}c@{}}\texttt{COCO-} \\ \texttt{spatial}\end{tabular} & \begin{tabular}{@{}c@{}}\texttt{GQA-} \\ \texttt{spatial}\end{tabular} & Avg\\
               & \multicolumn{2}{c}{$c > c' > c''$ or $c'' > c' > c$ $(\downarrow)$} \\
              Model & \hspace{15px}\texttt{REPLACE}\hspace{15px} & \texttt{SWAP} \\
              % Model & \begin{tabular}{@{}c@{}}$c > c' > c''$ \\ or \\$c'' > c' > c$\end{tabular} & \begin{tabular}{@{}c@{}}$c > c' > c''$ \\ or \\$c'' > c' > c$\end{tabular} \\
              \midrule
              CLIP ViT-B/32 & 23.2 & 21.7\\
              \midrule
              Our HN & 21.0 & 25.1\\
              Our HP+HN & 16.9 & 22.9\\
              Our HP+HN (Swap-only) & 18.6 & 21.2\\
              Our HP+HN (Replace-only) & 17.8 & 26.5\\
              \midrule
              Human Estimate &  & \\
              \bottomrule \\
            \end{tabular}
        }
\caption{Our brittleness is less.
}
\label{tab:improved_results_2}
\end{table}

% {\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}}97


==> tables/main_results_a.tex <==
\begin{table}[t]
\centering
\resizebox{0.65\columnwidth}{!}{  

            \begin{tabular}{lcccc}
            \toprule
              % Model & \begin{tabular}{@{}c@{}}\texttt{Whats-} \\ \texttt{Up}\end{tabular} & \begin{tabular}{@{}c@{}}\texttt{COCO-} \\ \texttt{spatial}\end{tabular} & \begin{tabular}{@{}c@{}}\texttt{GQA-} \\ \texttt{spatial}\end{tabular} & Avg\\
               & \multicolumn{2}{c}{\texttt{REPLACE}} & \multicolumn{2}{c}{\texttt{SWAP}} \\
              Model & \hspace{5px}$c > c_N$\hspace{5px} & \hspace{5px}$c, c_P > c_N$\hspace{5px} & \hspace{5px}$c > c_N$ \hspace{5px}& $c, c_P > c_N$\\
              \midrule
              CLIP ViT-B/32 & 61.6 & 46.8 {\scriptsize\textcolor{red}{(-14.9)}}& 60.5 & 49.6 {\scriptsize\textcolor{red}{(-10.9)}} \\
              \midrule
              NegCLIP & 68.6 & 52.1 {\scriptsize\textcolor{red}{(-16.6)}}& 70.9 & 56.7 {\scriptsize\textcolor{red}{(-14.2)}}\\
              CREPE-Swap & 63.5 & 50.4 {\scriptsize\textcolor{red}{(-13.1)}}& 70.6 & 56.7 {\scriptsize\textcolor{red}{(-13.9)}}\\
              CREPE-Replace \hspace{20px}& 73.7 & 53.9 {\scriptsize\textcolor{red}{(-19.8)}}& 71.1 & 57.7 {\scriptsize\textcolor{red}{(-13.4)}}\\
              SVLC & 76.6 & 44.5 {\scriptsize\textcolor{red}{(-32.1)}}& 72.4 & 61.6 {\scriptsize\textcolor{red}{(-10.9)}}\\
              % SVLC-Pos & 55.6 & 39.9 {\scriptsize\textcolor{red}{(-15.7)}}& 52.0 & 38.4 {\scriptsize\textcolor{red}{(-13.6)}}  \\
              SVLC+Pos & 64.3 & 45.0 {\scriptsize\textcolor{red}{(-19.3)}}& 56.5 & 45.4 {\scriptsize\textcolor{red}{(-11.1)}} \\
              DAC-LLM & 87.6 & 48.9 {\scriptsize\textcolor{red}{(-38.7)}} & 72.0 & 61.1 {\scriptsize\textcolor{red}{(-10.9)}} \\
              DAC-SAM & 86.9 & 55.9 {\scriptsize\textcolor{red}{(-31.0)}}& 69.5 & 56.5 {\scriptsize\textcolor{red}{(-13.0)}} \\
              % LaCLIP &  &  &  & \\
              \midrule
              Human Estimate &  & & & \\
              \bottomrule \\
            \end{tabular}
        }
\caption{Results of CLIP and hard negative finetuned versions of it on our benchmark: Models don't do as well as you think. $s(c|i)$ is represented as $c$ for brevity. \replace averages performance on Attributes and Relations; refer to Supplementary for details.
}
\label{tab:main_results_1}
\end{table}

% {\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}}97


==> tables/main_results_b.tex <==
\begin{table}[t]
\centering
\resizebox{0.55\columnwidth}{!}{  

            \begin{tabular}{lcc}
            \toprule
              % Model & \begin{tabular}{@{}c@{}}\texttt{Whats-} \\ \texttt{Up}\end{tabular} & \begin{tabular}{@{}c@{}}\texttt{COCO-} \\ \texttt{spatial}\end{tabular} & \begin{tabular}{@{}c@{}}\texttt{GQA-} \\ \texttt{spatial}\end{tabular} & Avg\\
               & \multicolumn{2}{c}{$c > c_N > c_P$ or $c_P > c_N > c$ $(\downarrow)$} \\
              Model & \hspace{15px}\texttt{REPLACE}\hspace{15px} & \texttt{SWAP} \\
              % Model & \begin{tabular}{@{}c@{}}$c > c' > c''$ \\ or \\$c'' > c' > c$\end{tabular} & \begin{tabular}{@{}c@{}}$c > c' > c''$ \\ or \\$c'' > c' > c$\end{tabular} \\
              \midrule
              CLIP ViT-B/32 & 23.2 & 21.7\\
              \midrule
              NegCLIP & 21.5 & 26.4\\
              CREPE-Swap & 19.8 & 26.0\\
              CREPE-Replace & 23.9 & 25.4\\
              SVLC & 39.9 & 20.8\\
              % SVLC-Pos & 29.3 & 26.8\\
              SVLC+Pos & 29.8 & 22.8\\
              DAC-LLM & 40.1 & 21.6 \\
              DAC-SAM & 32.5 & 25.6\\
              % LaCLIP &  &  \\
              \midrule
              Human Estimate &  & \\
              \bottomrule \\
            \end{tabular}
        }
\caption{Results of CLIP and hard negative finetuned versions of it on our benchmark: Hard negative finetuning makes models brittle. $s(c|i)$ is represented as $c$ for brevity.
}
\label{tab:main_results_2}
\end{table}

% {\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}}97

